Schedulability Bounds for Parallel Real-Time Tasks under Global Rate-Monotonic Scheduling

Schedulability bounds not only serve as efficient tests to decide schedulability of real-time task systems but also reveal insights about the worst-case performance of scheduling algorithms. Different from sequential real-time task systems for which utilization is a suitable metric to develop schedulability bounds, schedulability of parallel real-time tasks depends on not only utilization but also the workload graph structure of tasks, which can be well represented by the tensity metric. In this paper, we develop new analysis techniques for parallel real-time task systems under Global Rate-Monotonic (G-RM) scheduling and obtain new results on schedulability bounds based on these two metrics: utilization and tensity. First, we develop the first utilization-tensity bound for G-RM. Second, we improve the capacity augmentation bound of G-RM from the best known value 3.73 to 3.18. These schedulability bounds not only provide theoretical insights about real-time performance of G-RM, but also serve as highly efficient schedulability tests, which are particularly suitable to design scenarios in which detailed task graph structures are unknown or may change at run-time. Experiments with randomly generated task sets show that our new results consistently outperform the state-of-the-art with a significant margin under different parameter settings.

==> overview.tex <==
%\subsection{Utilization-Based Bounds}




%
%Before go into the details, we first introduce some notations that is useful in the analysis.
%
%
%
%
%We denote by $S_{\infty,\gamma}$  the resulting schedule when $A_{\infty}$ schedules tasks on cores of speed $\gamma$, where $\gamma$ is the maximum elasticity, and $\gamma\leq 1$.  $S_{\infty,\gamma}$ finishes a job of task $\tau_i$ exactly $\frac{L_i}{\gamma}$ time units after it is released. Obviously, $S_{\infty,\gamma}$ is always feasible.
%
%
%
%
%\begin{lemma}\label{lem:key}
%	For any algorithm $A$ and a time interval $I = [t^*,t^{\times}]$, if the resulting schedule $S$ of $A$ does more than $S_{\infty,\gamma}$ before $t^*$, and $S$ fails at time $t^{\times}$, then during the interval $I$, the schedule  $S$  does at least $ (m  -\gamma(m-1))|I|$ units of workload.
%	\end{lemma}
%	
%	\begin{proof}
%		We now prove this lemma on the amount of workload done by $S$ in $I$.  Under algorithm $A$, we denote by $X$ the total length of the intervals within $I$ where  all $m$ cores are busy. Define $Y = |I| - X$. In the following, we show that $Y < \gamma |I|$. Otherwise, we assume that $ Y \geq \gamma |I| $. Denote by $Y_1,\cdots,Y_l \subseteq I$ all subintervals of $I$ where not all cores are busy. We define $t'$ such that $| [t^*,t'] \cap \cup_j Y_j | = \gamma (\lceil t^* \rceil - t^*)$. During all points in time within $[t^*,t'] \cap \cup_i Y_i$  all jobs that are available for $A$ may be scheduled in $S_{\infty,\gamma}$ during $[t^*,\lceil t^* \rceil ]$. Since during all these points in time $S$ does not use all cores, by time $t'$ it has processed at least as much of every job as $S_{\infty,\gamma}$ by time $\lceil t^* \rceil$.
%		
%		Next, define time points $t_i$, $i = 0,\cdots, t^{\times} - \lceil t^* \rceil$ such that $| [t^*,t_i] \cap \cup_j Y_j | = \gamma (\lceil t^* \rceil - t^* + i )$ for each $i$. We prove by induction that up to time $t_i$ the schedule $S$ has processed as much of every job as $S_{\infty,\gamma}$ by time $\lceil t^* \rceil +i$. The case $i = 0$ was proven above. Now suppose that the claim is true for some value $i$. Then at each time point during $[t^*,t_i] \cap \cup_j Y_j$ all jobs that are available for $S$ may be scheduled in $S_{\infty,\gamma}$ during $[ \lceil t^* \rceil +i, \lceil t^* \rceil + i +1  ]$. Since during all these time points $S$ does not use all cores, by time $t_{i+1}$, it has processed at least as much of every job as $S_{\infty,\gamma}$ by time $\lceil t^* \rceil +i +1$. By induction the claim is true for $i^* = t^{\times} - \lceil t^* \rceil$ and hence at time $\lceil t^* \rceil +i^* = t^{\times}$ the schedule $S$ has finished as much of every job as $S_{\infty,\gamma}$. This yields a contradiction since $S_{\infty,\gamma}$ is feasible and $S$ is not.
%		
%		Therefore, $ Y < \gamma |I|$. Hence, in the interval $I$ the schedule $S$ finishes at least
%		\begin{eqnarray}
%		 m X + Y & = &  m (|I| - Y) +  Y \nonumber \\
%		& = & m |I| - m Y +  Y \nonumber \\
%		& = &  m |I| -  Y (m-1) ~~~~[\because m>1] \nonumber \\
%		& >  &   m |I| - \gamma (m-1) |I| \nonumber
%		\end{eqnarray}
%		units of workload. 
%		\end{proof}


